A Bilingual, OpenWorld Video Text Dataset and End-to-end Video Text Spotter with Transformer

Most existing video text spotting benchmarks focus on evaluating a single language and scenario with limited data. In this work, we introduce a large-scale, Bilingual, Open World Video text benchmark dataset(BOVText). There are four features for BOVText. Firstly, we provide 2,000+ videos with more than 1,750,000+ frames, 25 times larger than the existing largest dataset with incidental text in videos. Secondly, our dataset covers 30+ open categories with a wide selection of various scenarios, e.g., Life Vlog, Driving, Movie, etc. Thirdly, abundant text types annotation (i.e., title, caption or scene text) are provided for the different representational meanings in video. Fourthly, the BOVText provides bilingual text annotation to promote multiple cultures live and communication. Besides, we propose an end-to-end video text spotting framework with Transformer, termed TransVTSpotter, which solves the multi-orient text spotting in video with a simple, but efficient attention-based query-key mechanism. It applies object features from the previous frame as a tracking query for the current frame and introduces a rotation angle prediction to fit the multiorient text instance. On ICDAR2015(video), TransVTSpotter achieves the state-of-the-art performance with 44.1% MOTA, 9 fps. The dataset and code of TransVTSpotter can be found at github:com=weijiawu=BOVText and github:com=weijiawu=TransVTSpotter, respectively.

==> tables/table11.tex <==
\def\x{{$\footnotesize \times$}}
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c|ccc|ccc|ccc|c}
    \whline
	\multirow{2}*{$\rm Method$} &
	
	\multicolumn{3}{c}{ICDAR2013~\cite{karatzas2013icdar}(video,D)/\%}&
	
	\multicolumn{3}{c}{ICDAR2013~\cite{nguyen2014video}(image,D)/\%}&
	
	\multicolumn{3}{c|}{ICDAR2015~\cite{zhou2015icdar}(image,D)/\%} 
    &
    \multirow{2}*{FPS}
    
	\cr\cline{2-10}  
	
	
% 	\cr\cline{0-1}  
	~ &  Precision & Recall & F-score & Precision & Recall & F-score & Precision & Recall & F-score   \cr\shline \hline
	\hline
	Wang \textit{et al.}~\cite{wang2018robust} & 71.9 & 58.6
& 62.6 & - & - & - & - & - & - & - \cr\hline
    
    Wu \textit{et al.}~\cite{wu2015new} & 63.0 & 68.0 & 65.0 & - & - & - & - & - & - & - \cr\hline
    
    Yu \textit{et al.}~\cite{yu2021end} & \textbf{82.4 }& 56.4 & 66.9 & - & - & - & - & - & - & -\cr\hline
    
    Wei \textit{et al.}~\cite{feng2021semantic} & 75.5 & 64.1 & 69.3 & - & - & - & - & - & - & 9.6 \cr\hline
    
    TextBoxes~\cite{liao2017textboxes} & - & - & - & 88.0 & 83.0 & 85.0 & - & - & - & 1.5 \cr\hline
    
    
	
	SegLink~\cite{shi2017detecting} & - & - & - & 87.7 & 83.0 & 85.3 & 73.1 & 76.8 & 75.0 & 8.9 \cr\hline

    Mask Textspotter~\cite{lyu2018mask} & - & - & - &  88.6 &  \textbf{95.0} & \textbf{91.7} & \textbf{91.6} & 81.0 & 86.0 & 4.8 \cr\hline
    
    CharNet~\cite{xing2019convolutional} & - & - & - & - & - & - & 88.3 & \textbf{91.1} & \textbf{89.7}  &  - \cr\hline
	
	TransVTSpotter(ours) & 73.4 & \textbf{69.4} & \textbf{71.1} & \textbf{91.4} & 89.6 & 91.0 &  86.8 & 81.7 & 84.2 & \textbf{13.0} \cr\hline

     \whline
\end{tabular}
		

==> tables/table2.tex <==
\def\x{{$\footnotesize \times$}}
\scriptsize
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{l||c|c||c|c|c||c|c|c}
    \whline
	$\rm Method$ & $\rm MOTP$ & $\rm MOTA$ & $\rm ID_P$/\% & $\rm ID_R$/\% & ${\rm {ID_{F1}}}$/\% & $\rm GT$ & $\rm MT$ & $\rm ML$  \cr\shline \hline
	\hline
    EAST~\cite{zhou2017east} & 0.275 & -0.301 & 23.5 & 22.9 & 23.2 & 48321 & 20.1\% & 74.2\%\\
    PSENet~\cite{psenet} & 0.112 & 0.334 & 34.7 & 26.7 & 29.9 & 48321 & 26.4\% & 69.1\%\\
    DB~\cite{liao2020real} & 0.102 & 0.438 & 33.7 & 29.9 & \textbf{31.7} & 48321 & 30.1\% & 65.1\%\\
    
     \whline
\end{tabular}


==> tables/table4.tex <==
\def\x{{$\footnotesize \times$}}
% \footnotesize
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{c|ccc|c|cccc|c|c}
    \whline
	\multicolumn{4}{c|}{Detection Performance/\%} & \multicolumn{7}{c}{ Recognition Performance/\%}  
	\cr\cline{0-10}  
% 	\cr\cline{0-1}  
	\multirow{2}*{Method} & \multirow{2}*{Precision} & \multirow{2}*{Recall} & \multirow{2}*{F-score} & \multirow{2}*{Method} & \multicolumn{3}{c}{Pretrained} & \multicolumn{3}{|c}{Fine tuned}
	\cr\cline{6-11}
	~ & ~ & ~ & ~ & ~ & CH & AN & ALL & CH & AN & ALL
	\cr\shline \hline 
	\hline
	EAST~\cite{zhou2017east} & 52.2 & 38.1 & 44.1 & CRNN~\cite{shi2016end} & 26.0 & 32.1 & 23.2 & 33.2 & 47.1 & 38.6 \cr\cline{6-11}
	PSENet~\cite{psenet} & 74.3 & 65.2 & 69.5 & RARE~\cite{shi2016robust} & 25.2 & 34.2 & 23.5 & 35.6 & 45.7 & 40.2 
	\cr\cline{6-11}
	DB~\cite{liao2020real} & 77.2 & 64.5 & 70.3 & GRCNN~\cite{wang2017gated} & 23.1 & 39.8 & 26.7 & 35.6 & 49.2 & 40.3 
	
    \cr\hline

     \whline
\end{tabular}


==> tables/table6.tex <==
\def\x{{$\scriptsize \times$}}
\tiny
\begin{tabular}{l|ccc|cccc}
    \whline
	\multirow{2}*{}   &\multicolumn{3}{c|}{Languages}  
	 &  \multicolumn{4}{c}{Text Category}\cr\cline{2-8} ~ & English & Chinese & Alphanumeric & Caption Text & Scene Text & \textcolor[RGB]{96,177,87}{Title} & \textcolor[RGB]{96,177,87}{Others} \cr\shline \hline
	\hline
    
    Video & 842(45\%)  & 1521(82\%) & 1023(55\%) & 1523(82\%) & 1336(72\%) & 222(12\%) & 148(8\%)  \\
    
    Video Frames & 671,462(40\%) & 1,449,824(86\%) &775,021(46\%) & 1,327,382(79\%) & 930,359(55\%)& 167,011(10\%) & 116,914(7\%) \\
    
    Text Instances& 2,785,643(38\%) & 5,308,766(72\%) & 3,150,256(43\%) &
    3,296,101(39\%) & 3,981,574(52\%)& 291,690(4\%) & 364,613(5\%)
    \\
     \whline
\end{tabular}

